MME-CoT: Benchmarking Chain-of-Thought in Large Multimodal Models for Reasoning Quality, Robustness, and Efficiency

Answering questions with Chain-of-Thought (CoT) has significantly enhanced the reasoning capabilities of Large Language Models (LLMs), yet its impact on Large Multimodal Models (LMMs) still lacks a systematic assessment and in-depth investigation. In this paper, we introduce MME-CoT, a specialized benchmark evaluating the CoT reasoning performance of LMMs, spanning six domains: math, science, OCR, logic, space-time, and general scenes. As the first comprehensive study in this area, we propose a thorough evaluation suite incorporating three novel metrics that assess the reasoning quality, robustness, and efficiency at a fine-grained level. Leveraging curated high-quality data and a unique evaluation strategy, we conduct an in-depth analysis of state-of-the-art LMMs, uncovering several key insights: 1) Models with reflection mechanism demonstrate a superior CoT quality, with Kimi k1.5 outperforming GPT-4o and demonstrating the highest quality results; 2) CoT prompting often degrades LMM performance on perception-heavy tasks, suggesting a potentially harmful overthinking behavior; and 3) Although the CoT quality is high, LMMs with reflection exhibit significant inefficiency in both normal response and self-correction phases. We hope MME-CoT serves as a foundation for advancing multimodal reasoning in LMMs. Project Page: https://mmecot.github.io/

==> tab/stat.tex <==
% \begin{table}[t]
% \small
% \caption{\textbf{Key Statistics of \dataset}}
% \centering
% % \begin{center}
% \begin{tabular}{lc}
% \toprule
% \textbf{Statistic} & \textbf{Number} \\
% \midrule
% Total questions & 1130 \\
% \quad - Reasoning split & 837 (74.1\%) \\
% \quad \quad Multiple-choice questions & 431 \\
% \quad \quad Free-form questions & 406 \\
% \quad - Perception split & 293 (25.9\%) \\
% \quad \quad Multiple-choice questions & 275 \\
% \quad \quad Free-form questions & 18 \\
% \midrule
% Total essential step annotation & 3865 \\
% \quad - Total inference conclusion & 2667 \\
% \quad - Average inference conclusion & 3.2 \\
% \quad - Total image observation & 1198 \\
% \quad - Average image observation & 1.4 \\
% Reference image caption item & 1579 \\
% Average reference caption & 1.9 \\
% \midrule
% Number of unique images & 2380 \\
% Number of unique questions & 808 \\
% Number of unique answers & 271 \\
% \midrule
% Maximum question length & 477 \\
% Maximum answer length & 15 \\
% Average question length & 41.2 \\
% Average answer length & 1.2 \\
% \bottomrule
% \end{tabular}
% % \end{center}
% % \vspace{-0.6cm}
% \label{table:statistics}
% \end{table}

% \begin{table}[t]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \vskip -0.1in
% \end{table}
